How Far Have LLMs Come Toward Automated SATD Taxonomy Construction?

Technical debt refers to suboptimal code that degrades software quality. When developers intentionally introduce such debt, it is called self-admitted technical debt (SATD). Since SATD hinders maintenance, identifying its categories is key to uncovering quality issues. Traditionally, constructing such taxonomies requires manually inspecting SATD comments and surrounding code, which is time-consuming, labor-intensive, and often inconsistent due to annotator subjectivity. In this study, we investigated to what extent large language models (LLMs) could generate SATD taxonomies. We designed a structured, LLM-driven pipeline that mirrors the taxonomy construction steps researchers typically follow. We evaluated it on SATD datasets from three domains: quantum software, smart contracts, and machine learning. It successfully recovered domain-specific categories reported in prior work, such as Layer Configuration in machine learning. It also completed taxonomy generation in under two hours and for less than $1, even on the largest dataset. These results suggest that, while full automation remains challenging, LLMs can support semi-automated SATD taxonomy construction. Furthermore, our work opens up avenues for future work, such as automated taxonomy generation in other areas.

==> Makefile <==
#!/usr/bin/make -f

CP=cp
RM=rm -f
TARG=paper

.PHONY: all clean

all:$(TARG).pdf

.SUFFIXES: .pdf .tex .aux .bbl

.tex.pdf:
	@\
	aux=$(<:%.tex=%.aux);\
	$(CP) $$aux $$aux-;\
	platex $<;\
	echo ========;\
	diff -q $$aux $$aux- > /dev/null;\
	if [ $$? -eq 0 ]; then\
		echo No need for second compile.;\
	else\
		bibtex $$aux;\
		echo ========;\
		$(CP) $$aux $$aux-;\
		platex $<;\
		echo ========;\
		diff -q $$aux $$aux- > /dev/null;\
		if [ $$? -eq 0 ]; then\
			echo No need for third compile.;\
		else\
			platex $<;\
		fi;\
	fi;\
	$(RM) $$aux-
	$(RM) $(TARG).{aux,bbl,log,blg,cut,out,xcp,gz,xcp,run.xml,bcf}
	bash convert.sh

clean:
	$(RM) $(TARG).{pdf,aux,bbl,log,blg,cut,out,xcp,gz,xcp,run.xml,bcf}


==> section/background.tex <==
\section{Background} \label{background}



==> section/rq.tex <==
\section{Research Questions} \label{rq}

% To evaluate the effectiveness of our automatic SATD category generation method, we define the following two Research Questions (RQs):

% Define RQs
\newcommand{\RQone}{\textbf{(Category name alignment)} To what extent can our method generate category names that are semantically similar to those defined by humans?}
\newcommand{\RQtwo}{\textbf{(Category content alignment)} Are the comments assigned to the categories generated by our method consistent with those defined by humans?}
% \newcommand{\rqtwo}{How well do the SATD categories generated by the LLM perform as clusters?}
\newcommand{\RQthree}{\textbf{(Efficiency)} How much time and cost does our method require?}

\begin{enumerate}[label=\textit{RQ\arabic*}, leftmargin=*, align=left]
    \item \RQone
    \item \RQtwo
    \item \RQthree
\end{enumerate}
RQ1 and RQ2 aim to compare the taxonomy generated by our method with that created by humans.
RQ1 focuses on the similarity of category names, while RQ2 examines the consistency of the comments assigned to each category.
RQ3 assesses the practicality of our method by measuring the execution time and monetary cost (\ie, API fees for LLMs) required to generate the SATD categories.



% \noindent
% \textbf{RQ1: \RQone}

% \noindent
% This RQ investigates whether the category names generated by our method semantically similar to those defined by humans.
% % 我々は，人間が生成したカテゴリとLLMが生成したカテゴリの意味的な類似度をカテゴリ名の埋め込み表現同士のコサイン類似度をとることで取得する．

% \vspace{0.5em}
% \noindent
% \textbf{RQ2: \RQtwo}

% \noindent
% This RQ examines whether the SATD categories generated by the LLM exhibit sufficient cohesion and separation as clusters, in comparison to human-defined categories.  
% To this end, we quantitatively evaluate intra-category coherence and inter-category separability using inter-cluster variance and the Silhouette score.

% \vspace{0.5em}
% \noindent
% \textbf{RQ3: \RQthree}

==> table/RQ1/category_frequency.tex <==
% \begin{table}[b]
% \centering
% \caption{Frequencies of Category Generation}
% \label{category_frequency}
% \scriptsize
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llrrrrrr}
% \toprule
% \textbf{Domain} & \textbf{Level} &
% \textbf{0 times} & \textbf{1 time} & \textbf{2 times} & \textbf{3 times} & \textbf{4 times} & \textbf{5 or more times} \\
% \midrule
% Quantum     & Main & \textbf{2 (50.0\%)} & 0 (0.0\%)   & 0 (0.0\%)   & 0 (0.0\%)   & 0 (0.0\%)   & \textbf{2 (50.0\%)} \\
%             & Sub  & \textbf{3 (33.3\%)} & 1 (11.1\%)  & 0 (0.0\%)   & 1 (11.1\%)  & 1 (11.1\%)  & \textbf{3 (33.3\%)} \\
% \midrule
% Blockchain  & Main & \textbf{6 (100.0\%)}& 0 (0.0\%)   & 0 (0.0\%)   & 0 (0.0\%)   & 0 (0.0\%)   & 0 (0.0\%) \\
%             & Sub  & \textbf{20 (80.0\%)}& 1 (4.0\%)   & 0 (0.0\%)   & 1 (4.0\%)   & 1 (4.0\%)   & \textbf{2 (8.0\%)} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}[b]
\centering
\caption{Number of categories by match count $n$.}
\label{category_frequency}
\scriptsize
\renewcommand{\arraystretch}{1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll
  >{\columncolor{gray!25}}l
  l
  >{\columncolor{gray!25}}l}
\toprule
Dataset & Level &
$\bm{n=0}$ & $1 \leq n \leq 4$ & $\bm{n \geq 5}$ \\
\midrule
Quantum Software     & Main & \textbf{2 (50.0\%)} & 0 (0.0\%)             & \textbf{2 (50.0\%)} \\
                     & Sub  & \textbf{3 (33.3\%)} & 3 (33.3\%)            & \textbf{3 (33.3\%)} \\
\midrule
Smart Contracts      & Main & \textbf{6 (100.0\%)}& 0 (0.0\%)             & \textbf{0 (0.0\%)} \\
                     & Sub  & \textbf{20 (80.0\%)}& 3 (12.0\%)            & \textbf{2 (8.0\%)} \\
\bottomrule
\end{tabular}
}
\end{table}


==> table/RQ2/intra_inter.tex <==
% \begin{table}[t]
% \centering
% \caption{Evaluation of Cluster Structure}
% \label{tab:intra_inter}
% \scriptsize
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llrrrr}
% \toprule
% \textbf{Domain} & \textbf{Level} &
% \textbf{Intra (LLM)↓} & \textbf{Intra (Human)↓} &
% \textbf{Inter (LLM)↑} & \textbf{Inter (Human)↑} \\
% \midrule
% Quantum     & Main & \textbf{0.4997} & 0.5229 & \textbf{0.0615} & 0.0384 \\
%             & Sub  & \textbf{0.4366} & 0.4742 & \textbf{0.1247} & 0.0871 \\
% \midrule
% Blockchain  & Main & \textbf{0.6432} & 0.6663 & \textbf{0.0607} & 0.0372 \\
%             & Sub  & \textbf{0.5229} & 0.5489 & \textbf{0.1810} & 0.1545 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}


% \begin{table}[t]
% \centering
% \caption{Evaluation of Cluster Structure}
% \label{tab:intra_inter}
% \scriptsize
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{llrrrr}
% \toprule
% \textbf{Domain} & \textbf{Level} &
% \textbf{Intra (LLM)↓} & \textbf{Intra (Human)↓} &
% \textbf{Inter (LLM)↑} & \textbf{Inter (Human)↑} \\
% \midrule
% Quantum     & Main & \textbf{0.4965} & 0.5173 & \textbf{0.0590} & 0.0383 \\
%             & Sub  & \textbf{0.4336} & 0.4690 & \textbf{0.1219} & 0.0866 \\
% \midrule
% Blockchain  & Main & \textbf{0.6426} & 0.6660 & \textbf{0.0611} & 0.0369 \\
%             & Sub  & \textbf{0.5352} & 0.5500 & \textbf{0.1684} & 0.1528 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}



% with NO_CATEGORY
\begin{table}[t]
\centering
\caption{Cluster Intra- and Inter-Variance for Human- and LLM-Generated Categories. Intra ↓ indicates intra-cluster variance (lower is better), and Inter ↑ indicates inter-cluster variance (higher is better).}
\label{tab:intra_inter}
\scriptsize
\renewcommand{\arraystretch}{1}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{llrrrr}
\toprule
Dataset & Level &
\multicolumn{2}{c}{Intra ↓} & \multicolumn{2}{c}{Inter ↑} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & LLM & Human & LLM & Human \\
\midrule
Quantum Software     & Main & \textbf{0.49} & 0.52 & \textbf{0.06} & 0.04 \\
            & Sub  & \textbf{0.43} & 0.47 & \textbf{0.12} & 0.09 \\
\midrule
Smart Contracts  & Main & \textbf{0.64} & 0.67 & \textbf{0.06} & 0.04 \\
            & Sub  & \textbf{0.54} & 0.55 & \textbf{0.16} & 0.15 \\
\bottomrule
\end{tabular}
}
\end{table}



% without NO_CATEGORY
\begin{table}[t]
\centering
\caption{Cluster Intra- and Inter-Variance for Human- and LLM-Generated Categories. Intra ↓ indicates intra-cluster variance (lower is better), and Inter ↑ indicates inter-cluster variance (higher is better).}
\label{tab:intra_inter}
\scriptsize
\renewcommand{\arraystretch}{1}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{llrrrr}
\toprule
Dataset & Level &
\multicolumn{2}{c}{Intra ↓} & \multicolumn{2}{c}{Inter ↑} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & LLM & Human & LLM & Human \\
\midrule
Quantum Software     & Main & \textbf{0.50} & 0.52 & \textbf{0.06} & 0.04 \\
            & Sub  & \textbf{0.43} & 0.47 & \textbf{0.12} & 0.08 \\
\midrule
Smart Contracts  & Main & \textbf{0.64} & 0.67 & \textbf{0.06} & 0.04 \\
            & Sub  & \textbf{0.54} & 0.55 & \textbf{0.17} & 0.15 \\
\bottomrule
\end{tabular}
}
\end{table}


==> table/RQ2/quant_eval.tex <==
\begin{table}[b]
\centering
\caption{クラスタ構造としての評価}
\label{tab:quant_eval}
\scriptsize
\renewcommand{\arraystretch}{1.2}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llrrrr}
\toprule
\textbf{Domain} & \textbf{Level} &
\textbf{Silh (LLM)↑} & \textbf{Silh (Hum)↑} &
\textbf{Var (LLM)↓} & \textbf{Var (Hum)↓} \\
\midrule
Quantum   & Main  & \textbf{0.014} & -0.006 & \textbf{0.476} & 0.495 \\
          & Sub   & \textbf{-0.004} & -0.018 & \textbf{0.415} & 0.436 \\
\midrule
Smart Contract & Main  & \textbf{-0.007} & -0.022 & 0.602 & \textbf{0.521} \\
           & Sub   & \textbf{-0.020} & -0.026 & \textbf{0.493} & 0.504 \\
\bottomrule
\end{tabular}
}
\end{table}

==> table/RQ2/variance_comparison.tex <==
\begin{table}[t]
  \centering
  \caption{カテゴリごとの分散の例}
  \label{tab:variance_comparison}
  \scriptsize
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{lccc}
  \toprule
  \textbf{Category} & \textbf{Domain} & \textbf{Variance} & \textbf{Sample Count} \\
  \midrule
  System Integration        & Quantum      & 0.5550 & 29 \\
  Algorithm Implementation  & Quantum      & 0.5365 & 25 \\
  Circuit Optimization      & Quantum      & 0.4443 & 21 \\
  Noise Handling            & Quantum      & 0.3886 & 13 \\
  \midrule
  Memory Management         & Blockchain   & 0.6856 & 28 \\
  Data Storage              & Blockchain   & 0.6723 & 29 \\
  Access Control            & Blockchain   & 0.6694 & 31 \\
  Transaction Integrity     & Blockchain   & 0.6330 & 47 \\
  Error Handling            & Blockchain   & 0.6255 & 29 \\
  Gas Optimization          & Blockchain   & 0.5388 & 9  \\
  \bottomrule
  \end{tabular}
  }
  \end{table}
